Graphical Models for Discrete and Continuous Data

We introduce a general framework for undirected graphical models. It generalizes Gaussian graphical models to a wide range of continuous, discrete, and combinations of different types of data. The models in the framework, called exponential trace models, are amenable to estimation based on maximum likelihood. We introduce a sampling-based approximation algorithm for computing the maximum likelihood estimator, and we apply this pipeline to learn simultaneous neural activities from spike data.

==> Sections/FigGraph.tex <==

%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:


\begin{figure}[t]
  \centering
  \begin{minipage}[h]{0.3\linewidth}
~\\~\\
  $\tilde V=\{1,2,3,4\}$\\
$\tilde E=\{(1,2),(2,3)\}$\\
$\bar E=\{(1,2),(2,3),(1,3)\}$
  \end{minipage}
  \begin{minipage}[h]{0.30\linewidth}
  \begin{align*}
\matrix=    \begin{bmatrix}
    1.2 & - 0.2 & 0 & 0  \\
    - 0.2 & 1.5 & 0.1 &  0  \\
     0 & 0.1 & 1 &  0 \\
    0 & 0 & 0 & 0.5
\end{bmatrix}~~~~~~
  \end{align*}   
  \end{minipage}
  \begin{minipage}[t]{0.28\linewidth}
\begin{tikzcd}[%
    ,cells={nodes={circle,draw,font=\sffamily\footnotesize\bfseries}}
    ,every arrow/.append style={-,thick}
    ]
& 
1\arrow{dl}{}\arrow[dashed]{dr}{}%\arrow{dr}{}%\arrow[loop above, near end, "0.1"] 
& \\
%%%%%%%%%%%
2%\arrow[bend left]{ur}{0.3}\arrow{dr}{0.8}
& & 
3\arrow{ll}{} \\
%%%%%%%%%%%
& 
4\arrow[dashed]{ul}{}\arrow[dashed]{ur}{}%\arrow{ur}{0.2}\arrow[bend left]{ul}{0.1} 
& 
\end{tikzcd}
  \end{minipage}
  \caption{Example of a vertex set $\tilde V,$ edge set $E,$ and matrix $\matrix$  and the corresponding graph. We can derive from the graph for example that  $\data_1$ and $\data_4$ are dependent (indicated by $(1,4)\in\bar E$), but they are conditionally independent given the other elements of~\data\ (indicated by $(1,4)\notin E$). }
  \label{fig:graph}
\end{figure}



==> Sections/FigGraphCRF.tex <==

%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:


\begin{figure}[t]
  \centering
  \begin{minipage}[t]{0.2\linewidth}
      \begin{align*}
\matrix^1=    \begin{bmatrix}
    1 &  0.1\\
     0.1 & 1\\
\end{bmatrix}~~~~~~
  \end{align*}
  \end{minipage}
  \begin{minipage}[t]{0.2\linewidth}
\begin{tikzcd}[%
    ,cells={nodes={circle,draw,font=\sffamily\footnotesize\bfseries}}
    ,every arrow/.append style={-,thick}
    ]
& 
\ensuremath{Z=0}\arrow{dl}{}\arrow{dr}{}%\arrow{dr}{}%\arrow[loop above, near end, "0.1"] 
& \\
%%%%%%%%%%%
\ensuremath{Y_1}%\arrow[bend left]{ur}{0.3}\arrow{dr}{0.8}
& &\ensuremath{Y_2}
\end{tikzcd}
  \end{minipage}
  \begin{minipage}[t]{0.2\linewidth}
      \begin{align*}
\matrix^2=    \begin{bmatrix}
    1 & 0\\
     0 & 1\\
\end{bmatrix}~~~~~~
  \end{align*}
  \end{minipage}
  \begin{minipage}[t]{0.2\linewidth}
\begin{tikzcd}[%
    ,cells={nodes={circle,draw,font=\sffamily\footnotesize\bfseries}}
    ,every arrow/.append style={-,thick}
    ]
& 
\ensuremath{Z=1}\arrow{dl}{}\arrow{dr}{}%\arrow{dr}{}%\arrow[loop above, near end, "0.1"] 
& \\
%%%%%%%%%%%
\ensuremath{Y_1}%\arrow[bend left]{ur}{0.3}\arrow{dr}{0.8}
& &\ensuremath{Y_2}\arrow{ll}{}
\end{tikzcd}
  \end{minipage}
  \caption{Example of a conditional random field with $X=(Y_1,Y_2,Z)\tp.$ The coordinates $Y_1$ and $Y_2$ are conditionally independent for $Z=0$ but not for $Z=1.$}
  \label{fig:graph}
\end{figure}



==> Sections/FigPotGraph.tex <==

%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:



\begin{figure}[t]
  \centering
  \begin{minipage}[h]{0.35\linewidth}
\begin{align*}
M=    \begin{bmatrix}
    1.2 & - 0.2 & 0 & 0  \\
    - 0.2 & 1.5 & 0 &  0.1  \\
     0& 0 & 1 &  0 \\
    0 & 0.1 & 0 & 0.5
\end{bmatrix}
  \end{align*}   
  \end{minipage}
  \begin{minipage}[t]{0.3\linewidth}
\begin{tikzcd}[%
    ,cells={nodes={circle,draw,font=\sffamily\footnotesize\bfseries}}
    ,every arrow/.append style={-,thick}
    ]
    &
    1\arrow{dl}{}%\arrow{dr}{}%\arrow[loop above, near end, "0.1"] 
&  \\
%%%%%%%%%%%
2%\arrow[bend left]{ur}{0.3}\arrow{dr}{0.8}
& & 
3\arrow[dashed]{ll}{} \\
%%%%%%%%%%%
& 
4%\arrow{ur}{0.2}\arrow[bend left]{ul}{0.1} 
& 
\end{tikzcd}
  \end{minipage}
  \caption{An illustration of how $E$ captures the dependence structure among the variables. The total number of coordinates is here $\originaldim=4;$ the number of coordinates involved in the graph is $\newdim=3.$ The set \potentialset\ of potential edges contains two edges (continuous and dashed lines in graph); the function $\linkfunction$ provides the connection of these edges with the parameter vector $\corvec.$ The edge set finally contains one element (continuous line in the graph). The graph alone is sufficient to make the following two statements: $\data_1$ and $\data_2$ are conditionally dependent while $\data_1$ and $\data_3$ are conditionally independent given all other vertices. No statement can be made about the other connections.}
  \label{fig:graphnew2}
\end{figure}

==> Sections/FigPotGraph2.tex <==

%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:


\newcommand{\so}{4.4}
\newcommand{\ho}{0}
\newcommand{\dul}{ \hspace{-\so mm}\textcolor{white}{3~}}
\newcommand{\dur}{\textcolor{white}{~3} \hspace{-\so mm}}
\begin{figure}[t]
  \centering
  ~~~~~~\begin{minipage}[h]{0.45\linewidth}
\begin{align*}
\matrix=  \begin{bmatrix}
&&&&1\\
&&&&0\\
&&0_{p\times(p-1)}&&\vdots\\
    \\
&&&&0
  \end{bmatrix}~~~~~~~~~~~~
\end{align*}
  % \begin{align*}
%   \corvec=  \begin{bmatrix}
%     2\\ 
%   0\\
%    \vdots\\
%     0\\
% \end{bmatrix}~~~~~
%   \end{align*}
  \end{minipage}
  \begin{minipage}[t]{0.45\linewidth}
\begin{tikzcd}[%
    ,cells={nodes={circle,draw,font=\sffamily\footnotesize\bfseries}}
    ,every arrow/.append style={-,thick}
    ]
    &
    1\arrow{dl}{}%\arrow{dr}{}%\arrow[loop above, near end, "0.1"] 
&  \\
%%%%%%%%%%%
2%\arrow[bend left]{ur}{0.3}\arrow{dr}{0.8}
& 3\arrow[dashed]{u}{}&\dul\cdots\dur&p\arrow[dashed]{ull}{} 
\end{tikzcd}
  \end{minipage}
  \caption{An illustration of how $\matrix$ captures the dependence relations between $\data_1$ and the covariates $\data_2,\dots,\data_p.$ The potential edges are depicted as solid  and dashed lines: the solid line means that $X_1$ is conditionally dependent of $X_2;$ the dashed lines mean that $X_1$ is conditionally independent of all other covariates. No statement is made about the dependencies among the covariates $X_1$ through $X_{p-1}.$}
  \label{fig:graphnew2}
\end{figure}

==> Sections/Figures.tex <==
\pagebreak
\section{Tables and Figures}
% Poisson 

%\begin{figure}[h]
%	\label{Poisson_ROC}
%	\caption{The average ROC curves for Poisson data obtained over 50 random graphs. Each graph has 20 nodes and edges generated with a probability of 0.15. The precision matrix has 0 on the diagonal and 0.3 on the non-zero off-diagonal. Each graph is recovered by a sample of 250 observations.}
%	\begin{minipage}{\textwidth}
%		\centering
%		\includegraphics[width=0.5\textwidth]{./Figure/Poisson_random_graph_average_sampleSize250} 
%	\end{minipage}
%	\vskip-3ex
%\end{figure}
%
%\newpage

\begin{table}[h]
	\label{Poisson_delta_AUC_table}	
	\caption{The comparison of AUC of ROC curves for Poisson data under various scenarios. Each scenario is realized with 50 random graphs. Only the realizations with non-singular covariance matrix (i.e., effective trials) are used to calculate the average AUC.}
	\begin{tabular}{|l|l|l|l|l|l|l|}
		\hline
		\multirow{2}{*}{p} & \multirow{2}{*}{diag} & \multirow{2}{*}{off} & \multirow{2}{*}{sample size} & \multirow{2}{*}{effect trials} & \multicolumn{2}{l|}{delta AUC} \\ \cline{6-7} 
		&                       &                      &                              &                                & etm - gm  & etm - partial cor  \\ \hline
		20                 & 0                     & 0.2                  & 250                          & 50                             & 0.063     & 0.053              \\ \hline
		20                 & 0                     & 0.2                  & 500                          & 50                             & 0.039     & 0.028              \\ \hline
		20                 & 0                     & 0.3                  & 250                          & 50                             & 0.057     & 0.031              \\ \hline
		20                 & 0                     & 0.3                  & 500                          & 50                             & 0.026     & 0.009              \\ \hline
		20                 & 0                     & 0.5                  & 250                          & 50                             & 0.068     & 0.016              \\ \hline
		20                 & 0                     & 0.5                  & 500                          & 50                             & 0.036     & 0.001              \\ \hline
		20                 & -1                    & 0.2                  & 250                          & 50                             & 0.055     & 0.040               \\ \hline
		20                 & -1                    & 0.2                  & 500                          & 50                             & 0.040      & 0.024              \\ \hline
		20                 & -1                    & 0.3                  & 250                          & 50                             & 0.054     & 0.022              \\ \hline
		20                 & -1                    & 0.3                  & 500                          & 50                             & 0.024     & -0.002             \\ \hline
		20                 & -1                    & 0.5                  & 250                          & 37                             & 0.064     & -0.010              \\ \hline
		20                 & -1                    & 0.5                  & 500                          & 41                             & 0.024     & -0.028             \\ \hline
		20                 & -2                    & 0.2                  & 250                          & 49                             & 0.032     & 0.016              \\ \hline
		20                 & -2                    & 0.2                  & 500                         & 50                	               &0.005           &-0.011                    \\ \hline
		20                 & -2                    & 0.3                  & 250                          & 45                             & 0.017     & -0.019             \\ \hline
		20                 & -2                    & 0.3                  & 500                          & 48                             & -0.014    & -0.044             \\ \hline
		20                 & -2                    & 0.5                  & 250                          & 15                             & -0.019    & -0.098             \\ \hline
		20                 & -2                    & 0.5                  & 500                          & 20                             & -0.045    & -0.108             \\ \hline
	\end{tabular}
\end{table}

\newpage

%\begin{figure}[h]
%	\label{Poisson_delta_AUC_plot}
%	\caption{Visualization of the AUC table for Poisson}
%	\begin{minipage}{\textwidth}
%		\centering
%		\includegraphics[width=0.8\textwidth]{./Figure/Poisson_delta_AUC_plot} 
%	\end{minipage}
%\end{figure}
%
%\newpage

% Exponential

%\begin{figure}[h]
%	\label{Exponential_ROC}
%	\caption{The average ROC curves obtained for Exponential data over 50 random graphs. Each graph has 20 nodes and a precision matrix in the form of a strictly diagonally dominant matrix. The precision matrix has 1 on the diagonal. Each graph is recovered by a sample of 500 observations.}
%	\begin{minipage}{\textwidth}
%		\centering
%		\includegraphics[width=0.5\textwidth]{./Figure/Exponential_random_graph_average_sampleSize500} 
%	\end{minipage}
%\end{figure}
%
%\newpage

\begin{table}[h]
	\label{Exponential_delta_AUC_table}
	\caption{The comparison of AUC of ROC curves for Exponential data in various scenarios. Each scenario is realized with 50 random graphs. Only the realizations with non-singular covariance matrix (i.e., effective trials) are used to calculate the average AUC.}
	\begin{tabular}{|l|l|l|l|l|}
		\hline
		\multirow{2}{*}{p} & \multirow{2}{*}{sample size} & \multirow{2}{*}{effect trials} & \multicolumn{2}{l|}{delta AUC} \\ \cline{4-5} 
		&                              &                                & etm - gm  & etm - partial cor  \\ \hline
		20                 & 250                          & 50                             & 0.065     & 0.040               \\ \hline
		20                 & 500                          & 50                             & 0.047     & 0.029              \\ \hline
		50                 & 250                          & 50                             & 0.076     & 0.059              \\ \hline
		50                 & 500                          & 50                             & 0.057     & 0.041              \\ \hline
	\end{tabular}
\end{table}

\newpage

% Poisson-Bernoulli

%\begin{figure}[h]
%	\label{Bernoulli_Poisson_ROC}
%	\caption{The average ROC curves obtained for a mixture of Poisson-Bernoulli data over 50 random graphs. Each graph has 10 nodes of Poisson and 10 nodes of Bernoulli. The edges are generated with a probability of 0.15. The precision matrix has -1 on the diagonal and 0.2 on the non-zero off-diagonal. Each graph is recovered by a sample of 500 observations.}
%	\begin{minipage}{\textwidth}
%		\centering
%		\includegraphics[width=0.5\textwidth]{./Figure/Bernoulli_Poisson_random_graph_average_sampleSize500} 
%	\end{minipage}
%\end{figure}
%
%\newpage

\begin{table}[h]
	\label{Bernoulli_Poisson_delta_AUC_table}
	\caption{The comparison of AUC of ROC curves for a mixture of Bernoulli and Poisson data for various scenarios. Each scenario has 20 nodes (10 Bernoulli and 10 Poisson). The off-diagonal entry of the Bernoulli block is 0.5. Each scenario is realized with 50 random graphs. Only the realizations with non-singular covariance matrix (i.e., effective trials) are used to calculate the average AUC.}
	\begin{tabular}{|l|l|l|l|l|l|l|l|}
		\hline
		\multicolumn{1}{|c|}{\multirow{2}{*}{p}} & \multirow{2}{*}{diag\_pois} & \multirow{2}{*}{off\_pois} & \multirow{2}{*}{diag\_binary} & \multirow{2}{*}{sample size} & \multirow{2}{*}{effective trials} & \multicolumn{2}{l|}{delta AUC} \\ \cline{7-8} 
		\multicolumn{1}{|c|}{}                   &                             &                            &                               &                              &                                   & etm - gm  & etm - partial cor  \\ \hline
		20                                       & 0                           & 0.2                        & -1                            & 250                          & 50                                & 0.080     & 0.006              \\ \hline
		20                                       & 0                           & 0.2                        & -1                            & 500                          & 50                                & 0.069     & -0.009             \\ \hline
		20                                       & 0                           & 0.2                        & -2                            & 250                          & 49                                & 0.066     & -0.012             \\ \hline
		20                                       & 0                           & 0.2                        & -2                            & 500                          & 50                                & 0.078     & -0.006             \\ \hline
		20                                       & 0                           & 0.5                        & -1                            & 250                          & 49                                & 0.078     & 0.021              \\ \hline
		20                                       & 0                           & 0.5                        & -1                            & 500                          & 50                                & 0.055     & 0.015              \\ \hline
		20                                       & 0                           & 0.5                        & -2                            & 250                          & 44                                & 0.089     & 0.030              \\ \hline
		20                                       & 0                           & 0.5                        & -2                            & 500                          & 47                                & 0.073     & 0.017              \\ \hline
		20                                       & -1                          & 0.2                        & -1                            & 250                          & 49                                & 0.132     & 0.011              \\ \hline
		20                                       & -1                          & 0.2                        & -1                            & 500                          & 50                                & 0.133     & 0.004              \\ \hline
		20                                       & -1                          & 0.2                        & -2                            & 250                          & 45                                & 0.119     & 0.000              \\ \hline
		20                                       & -1                          & 0.2                        & -2                            & 500                          & 47                                & 0.120     & -0.008             \\ \hline
		20                                       & -1                          & 0.5                        & -1                            & 250                          & 41                                & 0.123     & 0.018              \\ \hline
		20                                       & -1                          & 0.5                        & -1                            & 500                          & 47                                & 0.094     & 0.004              \\ \hline
		20                                       & -1                          & 0.5                        & -2                            & 250                          & 34                                & 0.115     & 0.007              \\ \hline
		20                                       & -1                          & 0.5                        & -2                            & 500                          & 40                                & 0.101     & 0.000              \\ \hline
		20                                       & -2                          & 0.2                        & -1                            & 250                          & 42                                & 0.130     & 0.003              \\ \hline
		20                                       & -2                          & 0.2                        & -1                            & 500                          & 47                                & 0.148     & -0.013             \\ \hline
		20                                       & -2                          & 0.2                        & -2                            & 250                          & 37                                & 0.135     & -0.008             \\ \hline
		20                                       & -2                          & 0.2                        & -2                            & 500                          & 42                                & 0.142     & -0.022             \\ \hline
		20                                       & -2                          & 0.5                        & -1                            & 250                          & 17                                & 0.046     & -0.046             \\ \hline
		20                                       & -2                          & 0.5                        & -1                            & 500                          & 27                                & 0.033     & -0.084             \\ \hline
		20                                       & -2                          & 0.5                        & -2                            & 250                          & 15                                & 0.072     & -0.042             \\ \hline
		20                                       & -2                          & 0.5                        & -2                            & 500                          & 23                                & 0.051     & -0.070             \\ \hline
	\end{tabular}
\end{table}

\newpage

%\begin{figure}[h]
%	\label{Bernoulli_Poisson_delta_AUC_plot}
%	\caption{Visualization of the AUC table for a mixture of Bernoulli and Poisson}
%	\begin{minipage}{\textwidth}
%		\centering
%		\includegraphics[width=0.8\textwidth]{./Figure/Bernoulli_Poisson_delta_AUC_plot} 
%	\end{minipage}
%\end{figure}
%
%\newpage

% Bernoulli-Gaussian

%\begin{figure}[h]
%	\label{Bernoulli_Gaussian_ROC}
%	\caption{The average ROC curves obtained for a mixture of Bernoulli-Gaussian observations over 50 random graphs. Each graph has 10 nodes of Gaussian and 10 nodes of Bernoulli. The edges are generated with a probability of 0.2. The precision matrix has -2 on the diagonal and 0.5 on the non-zero off-diagonal. Each graph is recovered by a sample of 250 observations.}
%	\begin{minipage}{\textwidth}
%		\centering
%		\includegraphics[width=0.5\textwidth]{./Figure/Bernoulli_Gaussian_random_graph_average_sampleSize250} 
%	\end{minipage}
%\end{figure}
%
%\newpage

\begin{table}[h]
	\label{Bernoulli_Gaussian_delta_AUC_table}
	\caption{The comparison of AUC of ROC curves for a mixture of Bernoulli and Gaussian data for various scenarios. Each scenario has 20 nodes. The Gaussian block of the parameter matrix is in the form of a strictly diagonally dominant matrix. The Gaussian block has 1 on the diagonal and 1/(max degree +1) on the other non-zero positions. The remaining part of the parameter matrix has the same diagonal entries, and non-zero off entry shown in the table, respectively. Each scenario is realized with 50 random graphs. Only the realizations with non-singular covariance matrix (i.e., effective trials) are used to calculate the average AUC.}
	\begin{tabular}{|l|l|l|l|l|l|l|l|}
		\hline
		\multirow{2}{*}{p} & \multirow{2}{*}{diag} & \multirow{2}{*}{off} & \multirow{2}{*}{ratio} & \multirow{2}{*}{sample size} & \multirow{2}{*}{effective trials} & \multicolumn{2}{l|}{delta AUC} \\ \cline{7-8} 
		&                       &                      &                        &                              &                                   & etm - gm   & etm - partialCor  \\ \hline
		20                 & -1                    & 1                    & 0.2                    & 150                          & 29                                & 0.005      & -0.08             \\ \hline
		20                 & -1                    & 1                    & 0.2                    & 250                          & 31                                & -0.029     & -0.11             \\ \hline
		20                 & -1                    & 1                    & 0.2                    & 500                          & 39                                & -0.056     & -0.115            \\ \hline
		20                 & -1                    & 1                    & 0.5                    & 150                          & 16                                & 0.018      & -0.079            \\ \hline
		20                 & -1                    & 1                    & 0.5                    & 250                          & 20                                & -0.032     & -0.114            \\ \hline
		20                 & -1                    & 1                    & 0.5                    & 500                          & 26                                & -0.07      & -0.139            \\ \hline
		20                 & -1                    & 1                    & 0.8                    & 150                          & 14                                & -0.015     & -0.057            \\ \hline
		20                 & -1                    & 1                    & 0.8                    & 250                          & 21                                & -0.037     & -0.073            \\ \hline
		20                 & -1                    & 1                    & 0.8                    & 500                          & 26                                & -0.069     & -0.081            \\ \hline
		20                 & -2                    & 0.5                  & 0.2                    & 150                          & 49                                & 0.001      & -0.059            \\ \hline
		20                 & -2                    & 0.5                  & 0.2                    & 250                          & 50                                & -0.01      & -0.068            \\ \hline
		20                 & -2                    & 0.5                  & 0.2                    & 500                          & 50                                & -0.012     & -0.055            \\ \hline
		20                 & -2                    & 0.5                  & 0.5                    & 150                          & 42                                & 0.049      & -0.045            \\ \hline
		20                 & -2                    & 0.5                  & 0.5                    & 250                          & 48                                & 0.025      & -0.059            \\ \hline
		20                 & -2                    & 0.5                  & 0.5                    & 500                          & 49                                & -0.007     & -0.069            \\ \hline
		20                 & -2                    & 0.5                  & 0.8                    & 150                          & 40                                & 0.059      & -0.005            \\ \hline
		20                 & -2                    & 0.5                  & 0.8                    & 250                          & 45                                & 0.035      & -0.016            \\ \hline
		20                 & -2                    & 0.5                  & 0.8                    & 500                          & 48                                & -0.005     & -0.03             \\ \hline
		20                 & -2                    & 1                    & 0.2                    & 150                          & 23                                & 0.037      & -0.065            \\ \hline
		20                 & -2                    & 1                    & 0.2                    & 250                          & 28                                & -0.003     & -0.104            \\ \hline
		20                 & -2                    & 1                    & 0.2                    & 500                          & 29                                & -0.04      & -0.121            \\ \hline
		20                 & -2                    & 1                    & 0.5                    & 150                          & 7                                 & 0.066      & -0.069            \\ \hline
		20                 & -2                    & 1                    & 0.5                    & 250                          & 10                                & 0.048      & -0.062            \\ \hline
		20                 & -2                    & 1                    & 0.5                    & 500                          & 15                                & -0.04      & -0.122            \\ \hline
		20                 & -2                    & 1                    & 0.8                    & 150                          & 9                                 & 0.024      & -0.056            \\ \hline
		20                 & -2                    & 1                    & 0.8                    & 250                          & 11                                & -0.008     & -0.072            \\ \hline
		20                 & -2                    & 1                    & 0.8                    & 500                          & 19                                & -0.056     & -0.080            \\ \hline
	\end{tabular}
\end{table}

\newpage

%\begin{figure}[h]
%	\label{Bernoulli_Gaussian_delta_AUC_plot}
%	\caption{Visualization of the AUC table for a mixture of Bernoulli and Gaussian}
%	\begin{minipage}{\textwidth}
%		\centering
%		\includegraphics[width=0.8\textwidth]{./Figure/Bernoulli_Gaussian_delta_AUC_plot} 
%	\end{minipage}
%\end{figure}
%
%\newpage

%\begin{figure}[h]
%	\label{Poisson_Gaussian_ROC}
%	\caption{The average ROC curves obtained for a mixture of Poisson-Gaussian observations over 50 random graphs. Each graph has 10 nodes of Gaussian and 10 nodes of Bernoulli. The edges are generated with a probability of 0.2. The precision matrix has -2 on the diagonal and 0.5 on the non-zero off-diagonal. Each graph is recovered by a sample of 250 observations.}
%	\begin{minipage}{\textwidth}
%		\centering
%		\includegraphics[width=0.5\textwidth]{./Figure/Poisson_Gaussian_random_graph_average_sampleSize250} 
%	\end{minipage}
%\end{figure}
%
%\newpage

\begin{table}[h]
	\label{Poisson_Gaussian_delta_AUC_table}
	\caption{The comparison of AUC of ROC curves for a mixture of Poisson and Gaussian data for various scenarios. Each scenario has 20 nodes. The Gaussian block of the parameter matrix is in the form of a strictly diagonally dominant matrix. The Gaussian block has 1 on the diagonal and 1/(max degree +1) on the other non-zero positions. The remaining part of the parameter matrix has the same diagonal entries, and non-zero off entry shown in the table, respectively. Each scenario is realized with 50 random graphs. Only the realizations with non-singular covariance matrix (i.e., effective trials) are used to calculate the average AUC.}
	\begin{tabular}{|l|l|l|l|l|l|l|}
	\hline
	p  & diag & off & ratio & sample size & AUC(etm) - AUC(precision) & AUC(etm) - AUC(partial cor) \\ \hline
	20 & 0    & 0.2 & 0.2   & 150         & 0.02                      & 0.003                       \\ \hline
	20 & 0    & 0.2 & 0.2   & 250         & 0.02                      & 0.006                       \\ \hline
	20 & 0    & 0.2 & 0.2   & 500         & 0.004                     & -0.004                      \\ \hline
	20 & 0    & 0.2 & 0.5   & 150         & 0.02                      & 0.002                       \\ \hline
	20 & 0    & 0.2 & 0.5   & 250         & 0.022                     & 0.002                       \\ \hline
	20 & 0    & 0.2 & 0.5   & 500         & 0.015                     & 0                           \\ \hline
	20 & 0    & 0.2 & 0.8   & 150         & 0.047                     & 0.032                       \\ \hline
	20 & 0    & 0.2 & 0.8   & 250         & 0.046                     & 0.029                       \\ \hline
	20 & 0    & 0.2 & 0.8   & 500         & 0.026                     & 0.01                        \\ \hline
	20 & 0    & 0.3 & 0.2   & 150         & 0.006                     & -0.009                      \\ \hline
	20 & 0    & 0.3 & 0.2   & 250         & -0.006                    & -0.015                      \\ \hline
	20 & 0    & 0.3 & 0.2   & 500         & -0.008                    & -0.011                      \\ \hline
	20 & 0    & 0.3 & 0.5   & 150         & 0.005                     & -0.012                      \\ \hline
	20 & 0    & 0.3 & 0.5   & 250         & -0.006                    & -0.023                      \\ \hline
	20 & 0    & 0.3 & 0.5   & 500         & -0.011                    & -0.018                      \\ \hline
	20 & 0    & 0.3 & 0.8   & 150         & 0.044                     & 0.019                       \\ \hline
	20 & 0    & 0.3 & 0.8   & 250         & 0.033                     & 0.011                       \\ \hline
	20 & 0    & 0.3 & 0.8   & 500         & 0.008                     & -0.002                      \\ \hline
	20 & -1   & 0.2 & 0.2   & 150         & 0.038                     & -0.011                      \\ \hline
	20 & -1   & 0.2 & 0.2   & 250         & 0.041                     & -0.013                      \\ \hline
	20 & -1   & 0.2 & 0.2   & 500         & 0.036                     & -0.014                      \\ \hline
	20 & -1   & 0.2 & 0.5   & 150         & 0.058                     & 0.001                       \\ \hline
	20 & -1   & 0.2 & 0.5   & 250         & 0.054                     & -0.015                      \\ \hline
	20 & -1   & 0.2 & 0.5   & 500         & 0.046                     & -0.018                      \\ \hline
	20 & -1   & 0.2 & 0.8   & 150         & 0.082                     & 0.044                       \\ \hline
	20 & -1   & 0.2 & 0.8   & 250         & 0.072                     & 0.021                       \\ \hline
	20 & -1   & 0.2 & 0.8   & 500         & 0.055                     & 0.005                       \\ \hline
	20 & -1   & 0.3 & 0.2   & 150         & 0.009                     & -0.04                       \\ \hline
	20 & -1   & 0.3 & 0.2   & 250         & -0.009                    & -0.054                      \\ \hline
	20 & -1   & 0.3 & 0.2   & 500         & -0.02                     & -0.046                      \\ \hline
	20 & -1   & 0.3 & 0.5   & 150         & 0.012                     & -0.046                      \\ \hline
	20 & -1   & 0.3 & 0.5   & 250         & 0.002                     & -0.059                      \\ \hline
	20 & -1   & 0.3 & 0.5   & 500         & -0.011                    & -0.057                      \\ \hline
	20 & -1   & 0.3 & 0.8   & 150         & 0.074                     & 0.019                       \\ \hline
	20 & -1   & 0.3 & 0.8   & 250         & 0.056                     & -0.002                      \\ \hline
	20 & -1   & 0.3 & 0.8   & 500         & 0.03                      & -0.012                      \\ \hline
	20 & -2   & 0.2 & 0.2   & 150         & 0.048                     & -0.031                      \\ \hline
	20 & -2   & 0.2 & 0.2   & 250         & 0.05                      & -0.044                      \\ \hline
	20 & -2   & 0.2 & 0.2   & 500         & 0.039                     & -0.058                      \\ \hline
	20 & -2   & 0.2 & 0.5   & 150         & 0.065                     & -0.015                      \\ \hline
	20 & -2   & 0.2 & 0.5   & 250         & 0.058                     & -0.048                      \\ \hline
	20 & -2   & 0.2 & 0.5   & 500         & 0.045                     & -0.072                      \\ \hline
	20 & -2   & 0.2 & 0.8   & 150         & 0.084                     & 0.02                        \\ \hline
	20 & -2   & 0.2 & 0.8   & 250         & 0.09                      & 0.004                       \\ \hline
	20 & -2   & 0.2 & 0.8   & 500         & 0.071                     & -0.027                      \\ \hline
	20 & -2   & 0.3 & 0.2   & 150         & 0.005                     & -0.079                      \\ \hline
	20 & -2   & 0.3 & 0.2   & 250         & -0.028                    & -0.12                       \\ \hline
	20 & -2   & 0.3 & 0.2   & 500         & -0.056                    & -0.13                       \\ \hline
	20 & -2   & 0.3 & 0.5   & 150         & 0.012                     & -0.087                      \\ \hline
	20 & -2   & 0.3 & 0.5   & 250         & -0.018                    & -0.131                      \\ \hline
	20 & -2   & 0.3 & 0.5   & 500         & -0.044                    & -0.14                       \\ \hline
	20 & -2   & 0.3 & 0.8   & 150         & 0.057                     & -0.02                       \\ \hline
	20 & -2   & 0.3 & 0.8   & 250         & 0.033                     & -0.058                      \\ \hline
	20 & -2   & 0.3 & 0.8   & 500         & 0.008                     & -0.071                      \\ \hline
\end{tabular}
\end{table}


\newpage

%\begin{figure}[h]
%	\label{Poisson_Gaussian_delta_AUC_plot}
%	\caption{Visualization of the AUC table for a mixture of Poisson and Gaussian}
%	\begin{minipage}{\textwidth}
%		\centering
%		\includegraphics[width=0.8\textwidth]{./Figure/Poisson_Gaussian_delta_AUC_plot} 
%	\end{minipage}
%\end{figure}







